Laplace Functional Ordering of Point Processes in Large-scale Wireless Networks

Stochastic orders on point processes are partial orders which capture notions like being larger or more variable. Laplace functional ordering of point processes is a useful stochastic order for comparing spatial deployments of wireless networks. It is shown that the ordering of point processes is preserved under independent operations such as marking, thinning, clustering, superposition, and random translation. Laplace functional ordering can be used to establish comparisons of several performance metrics such as coverage probability, achievable rate, and resource allocation even when closed form expressions of such metrics are unavailable. Applications in several network scenarios are also provided where tradeoffs between coverage and interference as well as fairness and peakyness are studied. Monte-Carlo simulations are used to supplement our analytical results.

==> figures.tex <==
\newpage

%\begin{figure}[tb]
%\begin{minipage}{1\textwidth}
%\centering
%\begin{center}
%\includegraphics[height=8.5cm,keepaspectratio]{images/Cellular_network.eps}
%\caption{Illustration of a cellular network. The red triangles represent base stations which form a stationary Poisson point process $\Phi_{\mathrm{B}}$ with intensity $\lambda_{\mathrm{B}}=0.1$ and the blue dots represent users which also form a stationary Poisson point process $\Phi_{\mathrm{M}}$ with intensity $\lambda_{\mathrm{M}}=1.0$.}
%\label{fig:System_model}
%\end{center}
%\end{minipage}
%\end{figure}
%
%\begin{figure}[tb]
%\begin{minipage}{1\textwidth}
%\centering
%\begin{center}
%\includegraphics[height=8.5cm,keepaspectratio]{images/Typical_cell.eps}
%\caption{Typical cell}
%\label{fig:Typical_cell}
%\end{center}
%\end{minipage}
%\end{figure}

%\begin{figure}[tb]
%\begin{minipage}{1\textwidth}
%\centering
%\begin{center}
%\includegraphics[height=8.5cm,keepaspectratio]{images/Tot_cell_cov_prob_PPP.eps}
%\caption{Total cell coverage probabilities}
%\label{fig:Tot_cell_cov_prob_PPP}
%\end{center}
%\end{minipage}
%\end{figure}

%\begin{figure}[tb]
%\begin{minipage}{1\textwidth}
%\centering
%\begin{center}
%%\includegraphics[height=8.5cm,keepaspectratio]{images/Cognitive_network_SUs.eps}
%\includegraphics[height=8.5cm,keepaspectratio]{images/Cognitive_network.eps}
%\caption{Illustration of a cognitive network. The red triangles represent base stations which form a stationary Poisson point process $\Phi_{\mathrm{B}}$ with intensity $\lambda_{\mathrm{B}}=0.1$ and the blue dots represent users which also form a stationary Poisson point process $\Phi_{\mathrm{M}}$ with intensity $\lambda_{\mathrm{M}}=1.0$.}
%\label{fig:Cognitive_network_SUs}
%\end{center}
%\end{minipage}
%\end{figure}

%\begin{figure}[tb]
%\begin{minipage}{1\textwidth}
%\centering
%\begin{center}
%\includegraphics[height=8.5cm,keepaspectratio]{images/CDF_SIR_cognitive_networks.eps}
%\caption{Non-singular path-loss models with different path-loss exponents, $\delta_1$ and $\delta_2$}
%\label{fig:CDF_SIR_cognitive_networks}
%\end{center}
%\end{minipage}
%\end{figure}
%
%\begin{figure}[tb]
%\begin{minipage}{1\textwidth}
%\centering
%\begin{center}
%\includegraphics[height=8.5cm,keepaspectratio]{images/Avg_rates_cognitive_networks.eps}
%\caption{Illustration of a cellular network. The red triangles represent base stations which form a stationary Poisson point process $\Phi_{\mathrm{B}}$ with intensity $\lambda_{\mathrm{B}}=0.1$ and the blue dots represent users which also form a stationary Poisson point process $\Phi_{\mathrm{M}}$ with intensity $\lambda_{\mathrm{M}}=1.0$.}
%\label{fig:Avg_rates_cognitive_networks}
%\end{center}
%\end{minipage}
%\end{figure}

